Multi-Prompt with Depth Partitioned Cross-Modal Learning

In recent years, soft prompt learning methods have been proposed to fine-tune large-scale vision-language pre-trained models for various downstream tasks. These methods typically combine learnable textual tokens with class tokens as input for models with frozen parameters. However, they often employ a single prompt to describe class contexts, failing to capture categories' diverse attributes adequately. This study introduces the Partitioned Multi-modal Prompt (PMPO), a multi-modal prompting technique that extends the soft prompt from a single learnable prompt to multiple prompts. Our method divides the visual encoder depths and connects learnable prompts to the separated visual depths, enabling different prompts to capture the hierarchical contextual depths of visual representations. Furthermore, to maximize the advantages of multi-prompt learning, we incorporate prior information from manually designed templates and learnable multi-prompts, thus improving the generalization capabilities of our approach. We evaluate the effectiveness of our approach on three challenging tasks: new class generalization, cross-dataset evaluation, and domain generalization. For instance, our method achieves a $79.28$ harmonic mean, averaged over 11 diverse image recognition datasets ($+7.62$ compared to CoOp), demonstrating significant competitiveness compared to state-of-the-art prompting methods.

==> figure_tex/cam_point.tex <==
\begin{figure*}
\begin{center}
 \includegraphics[width=1.0\linewidth]{figure/cam_and_point.pdf}
\end{center}
\vspace{-3.0cm}
\caption{Training pipeline}
 
\label{fig:cam_point}
\end{figure*}

==> figure_tex/first_cam.tex <==
\begin{figure}[htp]
\begin{center}
\vspace{0.3cm}
\includegraphics[width=0.8\linewidth]{figure/first_cam.pdf}
\end{center}
\vspace{-0.5cm}
\caption{The ScoreCAM of class of goldfinch}
\vspace{-0.5cm}
\label{fig:first_cam}
\end{figure}

==> table_tex/abaltion_cross_modal.tex <==
% \begin{table}[htbp]
%         \centering
%         \caption{Comparision with vallnilla multi-prompt model and CoOp-PLOT}
%         \begin{tabular}{lccc}
%             \toprule
%              & Base & New & H \\
%             \midrule
%             CLIP & 63.34 & \textbf{74.22} & 71.70 \\
%             CoOp & 82.69 & 63.22  & 71.66 \\
%             CoOp+PLOT & 81.44 & 67.24 &  73.66\\
%             vallnilla multi-prompt (w/i M) & 81.22 & 73.23 & 77.27 \\
%             \midrule
%             PMPO & \textbf{82.91} & \textbf{75.95} & \textbf{79.27}\\
%             \midrule
%             \bottomrule
%         \end{tabular}
%         \label{tab:plot}
% \end{table}
\begin{table}[htbp]
  \vspace{-0.2cm}
  \caption{Effect of ensembling the manually-designed prompt on the base-to-new  generalization on $11$ datasets. $M$ means  the manually-designed prompt. H:Harmonic mean.}
  \centering
  
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{lcc|cc|cc}
    \toprule
    \multicolumn{1}{l}{} & \multicolumn{2}{c|}{Base}  & \multicolumn{2}{c|}{New}&  \multicolumn{2}{c}{H}  \\
    \cmidrule{2-7}
    \multicolumn{1}{l}{datasets} & \multicolumn{1}{c}{w/o M}  & \multicolumn{1}{c|}{w/i M}& \multicolumn{1}{c}{w/o M}& \multicolumn{1}{c|}{w/i M} & \multicolumn{1}{c}{w/o M} & \multicolumn{1}{c}{w/i M}  \\
     \midrule   
     Imagnet & \textbf{77.11} &76.94 &70.45 &\textbf{70.55} & \textbf{73.62} &73.60   \\
     Caltech101 & \text{98.34} & 98.04& 93.27 &\textbf{93.24} & \textbf{95.74} & 95.63   \\
     OxfordPets & 95.78 &\textbf{95.84} &\textbf{97.45} & 97.37 & \textbf{96.61} & 96.60   \\
     StanfordCars & \textbf{74.76} &74.16 &74.06 &\textbf{74.15} &\textbf{74.41} & 74.16 \\
     Flowers102 & 96.68 & \textbf{97.12}& 71.87&\textbf{73.85} & 83.36 & \textbf{83.89} \\
     Food101 & 90.52 & \textbf{90.58}&91.50 & \textbf{91.80} & 91.00 & \textbf{91.22} \\
     FGVCAircraft & 38.14  & \textbf{38.46} &34.95 & \textbf{35.99} &36.47 &\textbf{37.18} \\
     SUN397 & 81.54 &\textbf{81.71} &77.80 &\textbf{78.22} & 79.71& \textbf{79.85} \\
     DTD & \textbf{81.33} &80.21 &59.54 &\textbf{60.95} &68.75 &\textbf{69.27}  \\
     EuroSAT & 93.73 &\textbf{94.24} &78.14 &\textbf{81.85} & 85.23&\textbf{87.41}   \\
     UCF101 &  \textbf{85.06}&84.85 & 76.74&\textbf{77.64} &80.69 &\textbf{81.09} \\
     \midrule 
     Average & \textbf{83.01}&75.09 &82.91 &\textbf{75.95} &78.85 &\textbf{79.27}\\
    \midrule         
    \bottomrule
    \end{tabular}%
  \label{tab: ablation_m2}
\end{table}

==> table_tex/ablation_manual.tex <==
\begin{table*}[htbp]
  \centering
  \caption{}
    \setlength{\tabcolsep}{10pt}
    \begin{tabular}{ccccccccccccc}
    \toprule
     & \multicolumn{12}{c}{Dataset} \\
     \cmidrule{2-13}    
    & \rotatebox[origin=c]{90}{Imagnet} & \rotatebox[origin=c]{90}{Caltech101} & \rotatebox[origin=c]{90}{OxfordPets} & \rotatebox[origin=c]{90}{StanfordCars} & \rotatebox[origin=c]{90}{Flowers102} & \rotatebox[origin=c]{90}{Food101} & \rotatebox[origin=c]{90}{Aircraft} & \rotatebox[origin=c]{90}{SUN397} & \rotatebox[origin=c]{90}{DTD} & \rotatebox[origin=c]{90}{EuroSAT} & \rotatebox[origin=c]{90}{UCF101} & \rotatebox[origin=c]{90}{Average}    \\
    \midrule
    base w/o manual  & \\
    base w/i manual& \\
    \midrule
    new w/o manual& \\
    new w/i manual& \\
    \midrule
    H w/o manual& \\
    H w/i manual & \\
    
    \bottomrule
    \end{tabular}%
  \label{tab:ablation_manual}%
\end{table*}


==> table_tex/few_shot_classification.tex <==
\begin{table}[htbp]
  \caption{few-shot classification}
  \centering
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{lcccc|c}
    \toprule
    \multicolumn{1}{l}{datasets} & \multicolumn{1}{c}{CoOp}  & \multicolumn{1}{c}{CoCoOp}& \multicolumn{1}{c}{MaPle}& \multicolumn{1}{c|}{KgCoOp} & \multicolumn{1}{c}{PMPO} \\
     \midrule   
     Imagnet & 69.38 &70.55 & &70.19 &     \\
     Caltech101 & 94.44 & 94.98&  &94.65 & 94.60  \\
     OxfordPets & 91.30 &93.01&  & 93.20 & 91.68   \\
     StanfordCars & 72.73 & 69.10 & &71.98& \textbf{74.47}  \\
     Flowers102 & 91.14 & 82.56 & &90.69 & 87.97  \\
     Food101 & 82.58 & 86.64& & 86.59 & 83.75  \\
     FGVCAircraft & 33.18  & 30.87 & &32.47  & \textbf{33.64} \\
     SUN397 & 70.13 &70.50 & &71.79  & 69.89 \\
     DTD & 58.57 &54.79 & &58.31 &\textbf{60.17}   \\
     EuroSAT & 68.62 &63.83 & & 70.84 & \textbf{80.37}\\
     UCF101 &  77.41 &74.99 & & 78.40 &76.35  \\
     \midrule 
     Average & 73.59 &71.98 &  & 74.48 &\textbf{74.77} \\
    \midrule         
    \bottomrule
    \end{tabular}%
  \label{tab:few_shot}
\end{table}
